Lifelong Learning with Dynamically Expandable Networks

We propose a novel deep network architecture for lifelong learning which we refer to as Dynamically Expandable Network (DEN), that can dynamically decide its network capacity as it trains on a sequence of tasks, to learn a compact overlapping knowledge sharing structure among tasks. DEN is efficiently trained in an online manner by performing selective retraining, dynamically expands network capacity upon arrival of each task with only the necessary number of units, and effectively prevents semantic drift by splitting/duplicating units and timestamping them. We validate DEN on multiple public datasets under lifelong learning scenarios, on which it not only significantly outperforms existing lifelong learning methods for deep networks, but also achieves the same level of performance as the batch counterparts with substantially fewer number of parameters. Further, the obtained network fine-tuned on all tasks obtained significantly better performance over the batch models, which shows that it can be used to estimate the optimal network structure even when all tasks are available in the first place.

==> approach_old.tex <==
\begin{figure*}
\begin{center}
\hspace{-0.15in}
\includegraphics[height=3cm]{figure/concept_all.png}
\caption{\small \textbf{Incremental learning of a dynamically expandable network:} \textbf{Left:} \emph{Selective retraining.} DEN first identifies neurons that are relevant to the new tasks, and selectively retrain the network parameters associated with them. \textbf{Center:} \emph{Dynamic network expansion.} If the selective retraining fails to obtain desired loss below set threshold, we expand the network capacity in a top-down manner, while eliminating any neurons that are unnecessary using group-sparsity regularization. \textbf{Right:} \emph{Network split/duplication}. DEN calculates the drift $\rho_i^t$ for each unit to identify units that have drifted too much from their original values during training and duplicate them.}  
\label{incremental}
%\vspace{-0.1in}
\end{center}
\end{figure*}
\section{Incremental Learning of a Dynamically Expandable Network}
%\jt{add algorithm box to here. selective->split->add}
\setlength\parindent{6pt}
We consider the problem of incremental training of a deep neural network under the lifelong learning scenario, where unknown number of tasks with unknown distributions of training data arrive at the model in sequence. Specifically, our goal is to learn models for a sequence of $T$ tasks, $t=1,\hdots,t,\hdots,T$ for \emph{unbounded} $T$ where the task at time point $t$ comes with  training data $\mathcal{D}_t = \{\vct{x}_i, {y}_i\}_{i=1}^{N_t}$. While our method is generic to any kinds of tasks, for simplification, we only consider the binary classification task, that is, $y \in \{0,1\}$ for input feature $\vct{x} \in \reals^d$. It is the main challenge in the lifelong learning setting that all the previous training datasets up to $t-1$ are not available at the current time $t$ (only the model parameters for the previous tasks are accessible, if any). The lifelong learning agent at time $t$ aims to learn the model parameter $\mat{W}^t$ by solving following problem:
%tasks comes in a stream $(\mathcal{D}_1, \dots, \mathcal{D}_t, \dots, \mathcal{D}_T)$; here, $\mathcal{D}_t = \{\mat{X}_i, \vct{y}_i\}_{i=1}^{N_t}$ is a training dataset for each task $t$, where $\mat{X}^t\in\mathbb{R}^{N_t\times d}$ and $\vct{y}^t\in\{0, 1\}^{N_t}$ are features and labels for task $t$ respectively, where $d$ is the dimensionality of the input features, and $N_t$ is the number of samples for task $t$. We assume that at each learning stage for task $t$, we only have the model parameter trained on tasks task $1, \dots, T$ available, that is $\mat{W}^{t-1}$, but the data to train the model $(\mathcal{D}_1, \dots, \mathcal{D}_{t-1})$ is unavailable. The objective of lifelong learning is then to learn the parameter $\mat{W}^t$ at each task $t$ that minimizes the task-specific loss, given as follows:

\begin{equation}
\minimize_{\mat{W}^t}\mathcal{L}(\mat{W}^t; \mat{W}^{t-1}, \mathcal{D}_t) + \lambda \Omega(\mat{W}^t), \quad t=1,\hdots% \\
%\forall{t}\in\{1,\dots,T\}
\end{equation}

where $\mathcal{L}$ is task specific loss function, $\mat{W}^t$ is the parameter for task $t$, and $\Omega(\mat{W}^t)$ is the regularization (e.g. element-wise $\ell_2$ norm) to enforce our model $\mat{W}^t$ appropriately. In case of a neural network which is our primary interest, $\mat{W}^t=\{\mat{W}_l\}_{l=1}^L$ is the weight tensor.   
%, which in case the learner is a neural network is the weight tensor, and $\Omega(\mat{W}^t)$ is some regularization on the parameter, such as $\ell_2$-regularization. %such that there is some knowledge transfer from $\mat{W}^{t-1}$ to $\mat{W}^t$. One popular regularization is the Frobenius norm regularization on the different of the two parameters: $\Omega(\mat{W}^t, \mat{W}^{t-1} = \|\mat{W}^t - \mat{W}^{t-1}\|_2^2$. This regularization has an effect of preventing the model parameter for $t_{th}$ task from deviating too much from the model parameter at step $t$. This can better condition $\mat{W}^t$ and at the same time can solve the semantic drift problem, where the model learned at later stages do not work well on the tasks in early stages.

%[TODO polish below]
%As mentioned in the introduction, the challenge in training with the above objective is to 1) efficiently transfer knowledge obtained from the previous tasks from by leveraging $\mat{W}^{t-1}$, while also 2) learning an optimal solution for $\mat{W}^t$, and at the same time 3) prevent semantic drift on tasks $\{1, \dots, t-1\}$. 

To tackle these challenges of lifelong learning, we let the network to maximally utilize the knowledge obtained form the previous tasks, while allowing it to dynamically expand its capacity when the accumulated knowledge alone cannot sufficiently explain the new task. Figure~\ref{incremental} and Algorithm 1 describes our incremental learning process.



\begin{algorithm}
\footnotesize
\caption{Incremental Learning of a Dynamically Expandable Network}
\begin{algorithmic}
\STATE {\textbf Input:} Dataset $\mathcal{D} = (\mathcal{D}_1, \dots, \mathcal{D}_T)$, Thresholds $\tau$, $\sigma$
\STATE {\textbf Output:} $\mat{W}^T$
\FOR {$t ={1,\dots,T}$} 
\IF {$t = 1$}
	\STATE Train the network weights $\mat{W}^1$ using Eq.~\ref{l1}	
\ELSE
\STATE $\mat{W}^t = SelectiveRetraining(\mat{W}^{t-1})$ \COMMENT{Selectively retrain the previous network using Algorithm 2 %\jh{, but use Eq.5 instead Eq.3 to prevent large change}
}
\IF {$\mathcal{L}_t  > \tau$}
	\STATE $\mat{W}^t = DynamicExpansion(\mat{W}^t)$ \COMMENT{Expand the network capacity using Algorithm 3}
	%\STATE {\color{blue} $\mat{W}^t = Split(\mat{W}^t)$ \COMMENT{Split and duplicate the units using Algorithm 4}}
\ENDIF
\STATE $\mat{W}^t = Split(\mat{W}^t)$ \COMMENT{Split and duplicate the units using Algorithm 4 
%\jh{without obtaining $\mat{\widetilde{W}}^t$ process} 
}
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}
In following subsections, we describe each component of our incremental learning algorithm in detail: 1) Selective retraining, 2) Dynamic network expansion, and 3) Network split/duplication. 
%We describe the details of each method in following subsections.   
%\subsection{Incremental Lifelong Learning of a Deep Network.}
%\setlength\parindent{6pt}
%\vspace{-0.2in}
\paragraph{Selective Retraining.}
%One of the main challenge in lifelong learning is achieving efficiency in training time. 
A most naive way to train the model for a sequence of tasks would be retraining the entire model every time a new task arrives. However, such retraining will be very costly for a deep neural network. Thus, we suggest to perform selective retraining of the model, by retraining only the weights that are affected by the new task. Specifically, we train the network with $\ell_1$-regularization to promote sparsity in the weights, such that each neuron is connected to only few neurons in the layer below:

\begin{equation} \label{l1}
\minimize_{\mat{W}^t}\mathcal{L}(\mat{W}^t; \mat{W}^{t-1}, \mathcal{D}_t) + \mu \sum_{l=1}^L\|\mat{W}_l^t\|_1
\end{equation}

%\begin{equation} \label{l1}
%\minimize_{\mat{W}^t}\mathcal{L}(\mat{W}^t; \mat{W}^{t-1}, \mathcal{D}_t) + \sum_{l=1}^L \big( \mu_1\|\mat{W}_l^t\|_1 + \mu_2 \|\mat{W}_l^t\|_2 \big)
%\end{equation}

%\begin{equation} \label{l1}
%\min_{\{\mat{W}_l^t\}}\mathcal{L}(\{\mat{W}_l^t\}; \mathcal{D}_t) + \mu \sum_{l=1}^L\|\mat{W}_l^t\|_1
%\end{equation}
\noindent where $1$$\le$${l}$$\le$${L}$ denotes the $l_{th}$ layer of the network, $\mat{W}_l^t$ is the network parameter at layer $l$, and $\mu$ is the regularization parameter of the element-wise $\ell_1$ norm for sparsity on $\mat{W}$. For convolutional layers, we apply $(2,1)$-norm on the filters, to select only few filters from the previous layer.

We attend to the fact that $\ell_1$-regularization results in sparse connectivity among the neurons, and thus we can drastically reduce the computation overheads if we can focus on the subnetwork connected new task. To this end, when a new task $t$ arrives at the model, we first fit a sparse linear model to predict task $t$ using topmost hidden units of the neural network via solving the following problem:
%
%Our motivation is a bit different and focused on feature selection; 
%We attend to the fact that $\ell_1$-regularization results in sparse connectivity among the neurons, and thus we can select a subnetwork by selecting an output node of a multi-task neural network. When a new task $t$ arrives at the model, we first fit a sparse linear model to predict task $t$ using topmost units of the neural network, as in Figure~\ref{fig:selective} and in the following equation:
%
\begin{equation}
\minimize_{\mat{W}_{L,t}^t}\mathcal{L}(\mat{W}_{L,t}^t \, ; \mat{W}_{1:L-1}^{t-1}, \mathcal{D}_t) + \mu \|\mat{W}_{L,t}^t\|_1
\label{eq:topselect}
\end{equation}
where $\mat{W}_{1:L-1}^{t-1}$ denotes the set of all other parameters except $\mat{W}_{L,t}^t$.   
%
That is, we solve this optimization to obtain the connections between output unit $o_t$ and the hidden units at layer $L$-$1$ (fixing all other parameters up to layer $L$-$1$ as $\mat{W}^{t-1}$).
\eat{
\begin{figure}[t]
\begin{minipage}{0.5\textwidth}
\begin{center}
\includegraphics[height=3cm]{figure/selective.png}
%\vspace{-0.2in}
\caption{\small \textbf{Selective retraining.} \textbf{(Left:)} We first learn the parameter for the output unit $o_t$ using $\ell_1$-regularization, and then perform breadth-first search from those selected units to identify all network weights that are connected to $o_t$.  \textbf{(Right:)} Then, we retrain the selected subnetwork while maintaining all other weights to be fixed.}
%\vspace{-0.1in}
\label{fig:selective}
\end{center}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{algorithm}[ht]
\small
   \caption{Selective Retraining}
   \label{alg:selective}
\begin{algorithmic}
   \STATE {\bfseries Input:} Datatset $\mathcal{D}_t$, Previous parameter $\mat{W}^{t-1}$
   \STATE {\bfseries Output:} network parameter $\mat{W}^t$
   \STATE Initialize $l\leftarrow{L-1}$, $S = \{o_t\}$
   \STATE Solve Eq.~\ref{eq:topselect} to obtain $\mat{W}_{L,t}^t$
   \STATE Add neuron $i$ to $S$ if the weight between $i$ and $o_t$ in $\mat{W}_{L,t}^t$ is not zero.
   \WHILE {$l > 0$}
   \STATE Add neuron $i$ to $S$ if there exists some neuron $j \in S$ such that the weight between $i$ and $j$ is nonzero according to $\mat{W}^{t-1}$.
   \STATE $l\leftarrow{l-1}$
   \ENDWHILE
   \STATE Solve Eq.~\ref{eq:patialtrain} to obtain $\mat{W}_{S}^t$ 
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}
}
%
\noindent Once we build the sparse connection at this layer, we can identify all units and weights in the network that are affected by the training, while leaving the part of the network that are not connected to $o_t$ unchanged. Specifically, we perform breadth-first search on the network starting from those selected nodes, to identify all units (and input feature) that have paths to $o_t$. Then, we train only the weights of the selected subnetwork $S$, denoted as $\mat{W}_S^t$:

\eat{
\begin{equation}
\minimize_{ \mat{W}_S^t }\mathcal{L}( \mat{W}_S^t \ ; \mat{W}_{S^c}^{t-1}, \mathcal{D}_t) + \mu \| \mat{W}_S^t \|_2 
\label{eq:patialtrain}
\end{equation}
}

\begin{equation}
\minimize_{ \mat{W}_S^t }\mathcal{L}( \mat{W}_S^t \ ; \mat{W}_{S^c}^{t-1}, \mathcal{D}_t) + \mu \| \mat{W}_S^t \|_2 
\label{eq:patialtrain}
\end{equation}
%
%
%to obtain units in layers one layer below the output unit layer that are connected to the output unit $o_t$ for the given task $t$. Since these neurons have sparse connectivity to lower layer neurons, which in turn also have sparse connectivity, we can identify all units and weights that are affected by the training of the selected topmost units, while leaving the part of the network that are not connected to $o_t$ unchanged. Specifically, we perform breadth-first search on the network starting from those selected nodes, to identify all units (and input feature) that have paths to $o_t$ (See Algorithm~\ref{alg:selective}). After this search process is done, we will have identified all parameters that are affected by the selected tompost neurons, which results in a subnetwork of the original network that is smaller in size. Then we train this subnetwork with $\mathcal{D}_t$, as follows:
%

\begin{algorithm}[t]
\small
   \caption{Selective Retraining}
   \label{alg:selective}
\begin{algorithmic}
   \STATE {\bfseries Input:} Datatset $\mathcal{D}_t$, Previous parameter $\mat{W}^{t-1}$
   \STATE {\bfseries Output:} network parameter $\mat{W}^t$
   \STATE Initialize $l\leftarrow{L-1}$, $S = \{o_t\}$
   \STATE Solve Eq.~\ref{eq:topselect} to obtain $\mat{W}_{L,t}^t$
   \STATE Add neuron $i$ to $S$ if the weight between $i$ and $o_t$ in $\mat{W}_{L,t}^t$ is not zero.
   \FOR {$l = L-1,\dots, 1$}
   \STATE Add neuron $i$ to $S$ if there exists some neuron $j \in S$ such that $\mat{W}_{l,ij}^{t-1} \ne 0$.
   \ENDFOR
   \STATE Solve Eq.~\ref{eq:patialtrain} to obtain $\mat{W}_{S}^t$ 
\end{algorithmic}
\end{algorithm}

We use the element-wise $\ell_2$ regularizer since the sparse connections have been already established\footnote{We can add in $\ell_1$-norm here for further identification of necessary weights}. This partial retraining will result in lower computational overhead and also help with avoiding negative transfer, since neurons that are not selected will not get affected by the retraining process. Algorithm 2 describes the selective retraining process.


 %Such selective transfer is also reasonable in consideration of knowledge transfer, as tasks that are not highly related might use completely different high-level features, although generic features at the lower layer will still be shared.

%\begin{equation}
%\min_{\{\hat{\mat{W}}_l^t\}}\mathcal{L}(\{\hat{\mat{W}}_l^t\}; \mathcal{D}_t) + \mu \sum_{l=1}^L \|\hat{\mat{W}}_L^t\|_2 
%\label{eq:patialtrain}
%\end{equation}
%

%\begin{algorithm}
%   \caption{Selective Retraining}
%   \label{alg:selective}
%\begin{algorithmic}
%   \STATE {\bfseries Input:} Datatset $\mathcal{D}_t$, Previous model parameter $\mat{W}^{t-1}$
%   \STATE {\bfseries Output:} network parameter $\mat{W}^t$
%   \STATE Initialize $l\leftarrow{L}$, $\hat{\mat{W}}^t = \{\}$
%   \STATE Solve Eq.~\ref{eq:topselect} to obtain $\mat{W}_{L-1,t}^t$
%   \WHILE {$l > 0$}
%   \STATE Select $\vct{h}_{l-1}^{t-1}$ based on $\mat{W}_l^t$
%   \STATE Select $\hat{\mat{W}}_l^t$ based on $\vct{h}_{l-1}^{t-1}$ and $\vct{h}_{l}^{t-1}$
%   \STATE $\hat{\mat{W}}^t = \hat{\mat{W}}^t \cup \{\hat{\mat{W}}_l^t\}$
%   \STATE $l\leftarrow{l-1}$
%   \ENDWHILE
%   \STATE Solve Eq.~\ref{eq:patialtrain}
%\end{algorithmic}
%\end{algorithm}
%
%where $\hat{\mat{W}}_l^t$ is the parameter and $\hat{\vct{h}}_{l}^t$ is the activation of the subnetwork at layer $l$, respectively.  

 %For example, suppose that task $t$-$1$ is to classify images of \emph{car}, and task $t$ is to classify \emph{zebra}. In such a case, the current task should not affect the previous task.

%All the above $\ell_1$-regularized optimization problem can be solved using iterative soft thresholding of the weights, using proximal gradient method.
%See Figure~\ref{fig:selective} for more details.

\paragraph{Dynamic Network Expansion.}
In case where the new task is highly relevant to the old ones, or aggregated partial knowledge obtained from each task is sufficient to explain the new task, selective retraining alone will be sufficient for the new task. However, when the learned features cannot accurately represent the new task, additional neurons need to be introduced to the network, in order to account for the features that are necessary for the new task. Some existing work~\cite{zhou2012online,progressive} are based on a similar idea. However, they are either inefficient due to iterative training that requires repeated forward pass~\cite{zhou2012online}, or adds in constant number of units at each task $t$ without consideration of the task difficulty~\cite{progressive} and thus are suboptimal in terms of performance and network capacity utility. 
%Zhou et al.~\cite{zhou2012online} iteratively adds in a single neuron until the loss drops below certain threshold, and Progressive Network~\cite{progressive} adds in fixed number of neurons at each layer, for each task $t$. 

%To overcome these limitations, we instead propose an efficient way to dynamically decide how many neurons to add at which layer, for each task without repeated retraining of the network for each unit. 
%
%After the network is trained from scratch ($t=1$) or selective retraining, we first consider expanding the topmost layer of a network with a constant number of units, say $k$, by introducing new set of weight $\mat{W}_l^\mathcal{N}$. Then, the weight matrix at $l_{th}$ layer becomes $\mat{W}_l = [\mat{W}_l^{t-1}; \mat{W}_l^{\mathcal{N}}]$. This will result in expanding the set of units $\vct{h}_L^t$ at $L$ by introducing $k$ new units $\vct{h}_L^\mathcal{N}$ at layer $L$.
\eat{
\begin{equation}
\begin{aligned}
\vct{h}_L^{t-1} = f_l(\mat{W}_L^t\vct{h}_{L-1}+\vct{b}_L^{t-1}) \\
\vct{h}_L^\mathcal{N} = f_l(\mat{W}_L^\mathcal{N}\vct{h}_{L-1}+\vct{b}_L^t) \\
\vct{h}_L^t= [\vct{h}_L^{t-1}; \vct{h}_L^\mathcal{N}]
\label{expansion}
\end{aligned}
\end{equation}
}

To overcome these limitations, we instead propose an efficient way of using group sparse regularization to dynamically decide how many neurons to add at which layer, for each task without repeated retraining of the network for each unit. Suppose that we expand the $l_{th}$ layer of a network with a constant number of units, say $k$, inducing two parameter matrices expansions: $\mat{W}_{l}^t = [\mat{W}_{l}^{t-1}; \mat{W}_{l}^{\mathcal{N}}]$ and $\mat{W}_{l-1}^t = [\mat{W}_{l-1}^{t-1}; \mat{W}_{l-1}^{\mathcal{N}}]$ for outgoing and incoming layers respectively, where $\mat{W}^{\mathcal{N}}$ is the expanded weight matrix involved with added neurons.  
%for connections between $o_t$ and $k$ new neurons. 
Since we do not always want to add in all $k$ units (depending on the relatedness between the new task and the old tasks), we perform group sparsity regularization on the added parameters as follows:  
\begin{equation} 
\begin{aligned}
\minimize_{\mat{W}_l^\mathcal{N}}\mathcal{L}(\mat{W}_l^\mathcal{N} \ ; \mat{W}_l^{t-1}, \mathcal{D}_t) + \mu \|\mat{W}_l^\mathcal{N}\|_1 + \gamma \sum_{g} \|\mat{W}_{l,g}^\mathcal{N}\|_2
\end{aligned}
\label{groupsparsity}
\end{equation}

where $g\in\mathcal{G}$ is a group defined on the incoming weights for each neuron. For convolutional layers, we defined each group as the activation map for each convolutional filter. This group sparsity regularization was used in~\cite{wen2016learning} and ~\cite{alvarez2016learning} to find the right number of neurons for a full network, while we apply it to the partial network. Algorithm \ref{alg:expansion} describes the details on how expansion works.
\eat{
\begin{figure}[t]
\begin{minipage}{0.55\textwidth}
\begin{center}
%\begin{tabular}{c c c}
\includegraphics[height=2.5cm]{figure/addition.png}
%\vspace{-0.1in}
% &
%\includegraphics[height=3cm]{figure/splitting.png}\\
%(a) Dynamic Network Expansion & & (b) Network split/duplication \\
%\end{tabular}
\end{center}
\caption{\small \textbf{(a) Dynamic network expansion.} \textit{(Left:)}At step $t$, if $\mathcal{L}_t > \tau$, we first add in constant number of neurons at the topmost layer, and then retrain the newly introduced parameters with group sparsity on the units, to remove any unnecessary units.  \textit{(Right:)} We continue this process in a top-down manner, until the loss drops below the threshold, or reaching the bottommost layer.}
\label{fig:expansion}
\end{minipage}
\begin{minipage}{0.44\textwidth}
\begin{algorithm}[t]
\small
   \caption{Dynamic Network Expansion}
   \label{alg:expansion}
\begin{algorithmic}
   \STATE {\bfseries Input:} Datatset $\mathcal{D}_t$, Threshold $\tau$
   \STATE Perform Algorithm \ref{alg:selective} and compute $\mathcal{L}$\\
   Initialize $l\leftarrow{L-1}$
%      \vspace{0.1in}
   \WHILE {$\mathcal{L} > \tau$ and $l > 0$}
     \STATE Add $k$ units $\vct{h}^\mathcal{N}$ at layer $l$
     \STATE Solve Eq.~\ref{groupsparsity} and compute $\mathcal{L}$
     \STATE Remove useless units in $\vct{h}^\mathcal{N}$
     \STATE $l\leftarrow{l-1}$

   \ENDWHILE
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}
}
%Thus, by simply adding a fixed number of neurons at each layer and performing group sparsity on the weights, we can decide how many neurons to add at each layer. This group sparsity regularization was used in~\cite{deep-ssl} and ~\cite{deep-gs} to find the right number of neurons for a full network, while we apply it to the partial weight matrix.
%where $m$ is the layer to expand and $g\in\mathcal{G}$ is a group defined on the incoming weights for each neuron at ${l}_{th}$ layer. Thus, by simply adding a fixed number of neurons at each layer and performing group sparsity on the weights, we can decide how many neurons to add at each layer. This group sparsity regularization was used in~\cite{deep-ssl} and ~\cite{deep-gs} to find the right number of neurons for a full network, while we apply it to the partial weight matrix.

%However, we do not want to add in all $k$ units, since not all of them might be necessary, depending on the relatedness between the new task and the old tasks. How can we then dynamically choose how many units to add at each layer? Removing unnecessary units can be done by removing all incoming weights to them. This can be implemented using group sparsity regularization on $\mat{W}^\mathcal{N}$, while grouping each unit's incoming weights using $\ell_2$-norm, as follows:


%A partial weight matrix $\mat{W}_i^\mathcal{N}$ can be added to the network by an operation called $\it {add}$ to create a $\it{new}$ unit. If the $\it{new}$ units are added, The dimensionality of the network will expand to $[h_i^\mathcal{O}; h_i^\mathcal{N}]\in\mathbb{R}^{n_i+\Delta\mathcal{N}}$ and update $n_i = n_i+\Delta\mathcal{N}$ after the training\sj{Is this necessary?}. In this model, every time a unit is added to a layer except $h_0$ and $h_L$, $|h_{i-1}|+|h_i|$ parameters are added.  %This is basic concept of our incremental learning. Based on this, we will introduce some variations.


After selective retraining is done, the network checks if the loss is below certain threshold. If not, then at each layer we expand its capacity by $k$ neurons and solve for Eq.~\ref{groupsparsity}. Due to group sparsity regularization in Eq.~\ref{groupsparsity}, hidden units (or convolutional filters) that are deemed unnecessary from the training will be dropped altogether. We expect that from this dynamic network expansion process, the model captures new features that were not previously represented by $\mat{W}_l^{t-1}$ to minimize residual errors, while maximizing the utilization of the network capacity by avoiding to add in too many units. 


%To describe the expansion process step by step, our algorithm adds in the neuron in a top down manner (See Figure~\ref{fig:expansion}). After selective retraining is done, the network checks if the loss is below certain threshold, and then if not, then network tries to expand the network capacity at the layer before the output unit layer) with fixed number of neurons, while all other task layers remain fixed. After the training at each layer $l$ is done, due to group sparsity regularization in Eq.~\ref{groupsparsity}, hidden units that are deemed unnecessary from the training will be dropped altogether. Then, the same process is repeated at one layer below, until the loss drops below set threshold or $l=0$. Detailed algorithm is given in Algorithm~\ref{alg:expansion}.

 %When the expansion occur, the parameter $W_i$ for the $l_{th}$ layer changes into $\mat{W}_l^t = [\mat{W}_l^{t-1}; \mat{W}_l^\mathcal{N}] \in \mathbb{R}^{N_{l-1} \times (N_l+k)}$ and $\mat{W}_{l+1}^t = [\mat{W}_{l+1}^{t+1}; \mat{W}_{l+1}^\mathcal{N}] \in \mathbb{R}^{N_{l} \times (N_{l+1}+k)}$, where $k$ is the number of non-sparse units after the group-sparsity regularization. 


%\setlength\parindent{6pt}
%An important detail to note here is that the network timestamps all newly introduced hidden units with $t$, such that the previously learned task predictors do not use the newly introduced units, at test time. Use of timestamped units at inference time, is further described in Subsection~\ref{inference}. 
%
%\begin{minipage}{0.44\textwidth}

%\end{minipage}

\begin{algorithm}[t]
\small
   \caption{Dynamic Network Expansion}
   \label{alg:expansion}
\begin{algorithmic}
   \STATE {\bfseries Input:} Datatset $\mathcal{D}_t$, Threshold $\tau$
   \STATE Perform Algorithm \ref{alg:selective} and compute $\mathcal{L}$\\
   \IF {$\mathcal{L} > \tau$}
	   \STATE Add $k$ units $\vct{h}^\mathcal{N}$ at all layers
	   \STATE Solve for Eq.~\ref{groupsparsity} at all layers
   \ENDIF
   \FOR {$l = L-1,\dots, 1$}
     \STATE Remove useless units in $\vct{h}^\mathcal{N}_l$
   \ENDFOR
%   \vspace{0.05in}
\end{algorithmic}
\end{algorithm}

\paragraph{Network Split/Duplication.}
A crucial challenge in lifelong learning is the problem of \emph{semantic drift}, or \emph{catastrophic forgetting}, which describes the problem where the model gradually fits to the later learned tasks and thus forgets what it learned for earlier tasks, resulting in degenerate performance for them. The most popular yet simple way of preventing semantic drift is to regularize the parameters from deviating too much from its original values using $\ell_2$-regularization, as follows:%One simple solution is to separate hidden neurons for tasks and only allow incoming weights from earlier to later tasks, as in~\cite{progressive}. Yet, this will prevent the models for the earlier learned tasks from benefiting from the knowledge obtained for later tasks. The selective retraining and network expansion process will allow the later learned tasks to affect the earlier learned tasks, as old parameters will be updated from the training with new data; however, this makes our model to be susceptible to semantic drift.


%to prevent such semantic drift is to fix the parameter for $\mat{W}^{t-1}$ and only solve for the newly added part $\mat{W}^t$, while allowing incoming weights from $\mat{W}^{t-1}$ to $\mat{W}^t$. This is the approach taken by Progressive network~\cite{progressive}. Yet, this will prevent the models for the earlier learned tasks from benefiting from the knowledge obtained for later tasks. (e.g. Earlier learned tasks have fewer examples and later, relevant tasks come with a lot of training data). The selective retraining and network expansion process will allow the later learned tasks to affect the earlier learned tasks, as old parameters will be updateFd from the training with new data; however, this makes our model to be susceptible to semantic drift.
%Also, since we use selective retraining as our base training method, we consider approaches that can prevent semantic drift while allowing to retrain the previous model parameters.
 

%{\color{red} $\ell_2$ square is used here; what about in (3)? just $\ell_2$?} 
\begin{equation}
\begin{aligned}
\min_{\mat{W}^t}\mathcal{L}(\mat{W}^t; \mathcal{D}_t ) + \lambda \|\mat{W}^t - \mat{W}^{t-1}\|_2^2
\end{aligned}
\label{eq:l2regular}
\end{equation} 
 where $t$ is the current task, and $\mat{W}_l^{t-1}$ is the weight tensor of the network trained for tasks $\{1, \dots, t-1\}$, and $\lambda$ is the regularization parameter. This $\ell_2$ regularization will enforce the solution $\mat{W}^t$ to be found close to $\mat{W}^{t-1}$, by the degree given by $\lambda$; if $\lambda$ is small, then the network will be learned to reflect the new task more while forgetting about the old tasks, and if $\lambda$ is high, then $\mat{W}^t$ will try to preserve the knowledge learned at previous tasks as much as possible. Rather than placing simple $\ell_2$ regularization, it is also possible to weight each element with Fisher information, as in~\cite{kirkpatrick2017overcoming}. Nonetheless, if number of tasks is large, or if the later tasks are semantically disparate from the previous tasks, it might become difficult to find a good solution for both previous and new tasks.

%However, one critical limitation of this approach is that to prevent semantic drift, the model should sacrifice the performance for the new tasks, as the parameter cannot change much to reflect the new knowledge  required to represent the new tasks. To overcome such limitation, \citet{ewc} proposes Elastic Weight Consolidation (EWC), which replaces the $\ell_2$-regularization(eq 3) with $\frac{\lambda}{2}\sum_i F_i\|\mat{W}^t - \mat{W}^{t-1}\|_2^2$, where $F_i$ is the $i_{th}$ diagonal entry of the Fisher information matrix~\cite{nnn}. The Fisher information matrix $\mat{F}$ basically consists of the square of the gradient for each parameter, at each iteration. %hence, EWC can consider both the amount of change at the current step, and and the amount of change between $t$ and $t$-$1$, for each parameter $w_i$. %\sj{Describe EWC in detail, including the regularization term and the description of the Fisher information matrix.}. 
%Intuitively, EWC allows to find the solution that is optimal for both the previous tasks and the current task, by varying the degree of regularization for each neuron, such that it allows larger changes to direction of the optimal solution for the current task $t$. %\jt{Not only EWC find the solution by varying the degree of $\lambda$, but also $\ell_2$. see above describe of mine for EWC. EWC consider both the current amount of change and the amount of that has changed from $t-1$. i don't know why it can be better. it can be same by controlling a hyperparameter i think. the current changing is already considered by $\ell_2$, is'n it?}

 %For example, suppose that the model has learned a feature describing \emph{stripe} pattern, in an early task of recognizing \emph{fence}, and then it encounters a new task of recognizing \emph{zebra}. The EWC method then will try to find a feature describing both the stripe pattern for the fence and the zebra; however, this can results in performance degeneration since the stripe patterns in the two object classes are quite different, as the former is artificial and the latter is natural. %., as this will expand the neuron instead of drifting it, and thus will effectively prevent semantic drift. 
\eat{
\begin{figure}[t]
\begin{minipage}{0.55\textwidth}
\begin{center}
\includegraphics[height=2.8cm]{figure/splitting.png}
%\vspace{-0.1in}
\caption{\small \textbf{Network split and duplication.} \textbf{(Left:)} We identify units which have significant drifted in their values in the course of selective retraining and network expansion. \textbf{(Right:)} Then, we split those neurons to create duplicates, which we timestamp in order to prevent them from being used by the old tasks.}
%\vspace{-0.15in}
\label{fig:split}
\end{center}
\end{minipage}
\begin{minipage}{0.44\textwidth}
\begin{algorithm}[H]
\small
   \caption{Network Split/Duplication}
   \label{alg2}
\begin{algorithmic}
	\STATE {\bfseries Input:} Weight $\mat{W}^{t-1}$, Threshold $\sigma$
	\STATE Perform Eq.~\ref{eq:l2regular} to obtain $\mat{\widetilde{W}}^t$
	\FOR{all hidden unit $i$}
		\STATE Compute $l_2$-distance $\rho_i^t$ for incoming weights of $i$ in $\mat{\widetilde{W}}^t$ and $\mat{W}^{t-1}$
   		   	\IF{$\rho_i^t < \sigma$}
   				\STATE Copy $i$ into $i'$
   			\ENDIF
	\ENDFOR
	\STATE Perform Eq.~\ref{eq:l2regular} with the initialization of $\mat{\widetilde{W}}^t$ to obtain $\mat{W}^t$
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}
}

A better solution in such a case, is to \emph{split} the neuron such that we have features that are optimal for two different tasks. After performing Eq. \ref{eq:l2regular}, we measure the amount of semantic drift for each hidden unit $i$,  $\rho_i^t$, as the $\ell_2$-distance  between the incoming weights at $t$-$1$ and at $t$. Then if $\rho_i^t > \sigma$, we consider that the meaning of the feature have significantly changed during training, and split this neuron $i$ into two copies (properly introducing new edges from and to duplicate). This operation can be performed for all hidden units in parallel. After this duplication of the neurons, the network needs to train the weights again by solving Eq. \ref{eq:l2regular} since \emph{split} changes the overall structure. However, in practice this secondary training usually converges fast due to the reasonable parameter initialization from the initial training. Algorithm 4 describes the algorithm for \emph{split} operation. 
  


%introducing a new weight $\vct{w}_j$, whose value is set to $\vct{w}_i^{t}$.     
%, by the cosine similarity $\vct{w}_i^t \vct{w}_i^{t-1} / \|\vct{w}_i^t\|\|\vct{w}_i^{t-1}\|$ between the old weight and the new weight, for each incoming weight to internal hidden unit $h_i$, over all training instances of the current task. Then, if $\vct{w}_i^t \vct{w}_i^{t-1} / \|\vct{w}_i^t\|\|\vct{w}_i^{t-1}\| > \sigma$, where $\sigma$ is some set threshold, then we consider that the content of the features might have significantly changed during the course of training, and split the neurons by introducing a new weight $\vct{w}_j$, whose value is set to $\vct{w}_i^{t}$. We further timestamps the duplicated units with task $t$, to block them from being used by the old tasks, to prevent further semantic drift. See Figure~\ref{fig:split} for more details. The new parameter $\vct{w}_j$ is also represented as a group of parameters that connected from an input to a single output unit. In Algorithm \ref{alg2}, we describe splitting process with $\vct{w}_j$ as a $\mat{W}^t_l[:, j]$, where $\mat{W}^t$ is parameter retrained for the current task $t$ and $\mat{W}^{t-1}$ is the parameter from the previous learning stage.

%\sj{Describe the splitting process in detail, and add an illustration that explains this process. Try to be as detailed as possible} \sj{Also, why do we need to retrain the network? We can simply copy the value of the parameter at $t_{th}$ step to be the value of the split neuron, since we have already trained it to see the difference between the two network\rq{}s parameters.}


%\setlength\parindent{6pt}

   
%In this phase, the weights for the original units will not deviate too much from the previous weights at $t$-$1$ due to the regularization while duplicated units are allowed to freely describe the new knowledge on task $t$ without regularization. 
%since the weights are initialized from their optimal values. From this splitting process, the original units can remember knowledge about the previous tasks and that the duplicated neurons can describe the new knowledge about the new task, while still benefiting from the previous knowledge as it is initialized from, and regularized with, the incoming weights of the neuron for previous tasks. %Also, this process is more efficient than the add procedure, since the network can decide how many neurons to add at a time.


%After adding the hidden units by this \emph{split} operation, the network further trains the weights to get the optimal solution for weights connected to duplicated units, since at this point they have more number of connections. However, in practice this secondary training converges fast since the weights are initialized from their optimal values. From this splitting process, the original units can remember knowledge about the previous tasks and that the duplicated neurons can describe the new knowledge about the new task, while still benefiting from the previous knowledge as it is initialized from, and regularized with, the incoming weights of the neuron for previous tasks. %Also, this process is more efficient than the add procedure, since the network can decide how many neurons to add at a time.
%. It is more efficient because agent decide how much to add at one time instead of adding units one at a time. 

%In the experiment section, we empirically show that our neuron splitting approach is superior to EWC in~\cite{ewc}, which starts to fail after certain iterations on datasets with large variations among tasks.

%if there is little relatedness between the learned tasks. 

%\setlength\parindent{6pt}

\begin{algorithm}[t]
\small
   \caption{Network Split/Duplication}
   \label{alg:spdupl}
\begin{algorithmic}
	\STATE {\bfseries Input:} Weight $\mat{W}^{t-1}$, Threshold $\sigma$
	\STATE Perform Eq.~\ref{eq:l2regular} to obtain $\mat{\widetilde{W}}^t$
	\FOR{all hidden unit $i$}
%		\STATE $\rho_i^t = sim(\vct{w}_i^t, \vct{w}_i^{t-1})$    	
		\STATE $\rho_i^t = \|\vct{w}_i^t - \vct{w}_i^{t-1}\|_2$
   		   	\IF{$\rho_i^t >           \sigma$}
   				\STATE Copy $i$ into $i'$
   			\ENDIF
	\ENDFOR
	\STATE Perform Eq.~\ref{eq:l2regular} with the initialization of $\mat{\widetilde{W}}^t$ to obtain $\mat{W}^t$
%	\vspace{-0.02in}
\end{algorithmic}
\end{algorithm}

\paragraph{Timestamped Inference.}
\label{inference}
In both the network expansion and network split procedures, we timestamp each newly added unit $j$ by setting $\{\vct{z}\}_j=t$, which stores the training stage $t$ when it is added to the network, to more effectively prevent semantic drift caused by the introduction of new hidden units. At inference time, each task will only use the parameters that were introduced up to stage $t$, to prevent the old tasks from using new hidden units added in the training process. This is a more flexible strategy than fixing the weights learned up to each learning stage as in~\cite{rusu2016progressive}, since early tasks can still benefit from the learning at later tasks, via units that are further trained, but not split.
%\sj{Maybe we need an illustration}
\eat{
\begin{algorithm}[H]
\small
   \caption{Combined algorithm}
   \label{alg:combined}
\begin{algorithmic}
   \STATE {\bfseries Input:} Datatset $\mathcal{D}$, Threshold $\tau$, $\sigma$
   \STATE $T \leftarrow 0$, $\mat{W}^t \leftarrow$ initialize
   \WHILE {isMoreTask()}
   		\STATE $T \leftarrow T+1$
   		\STATE $\mathcal{D}_t \leftarrow$ getNextData()
   			\IF {$\mathcal{D}_t$ is first task}
   				\STATE solve $\minimize_{\mat{W}^t}\mathcal{L}(\mat{W}^t, \mathcal{D}_t) + \mu \|\mat{W}^t\|_1 + \gamma \|\mat{W}^t\|_2$
   			\ELSE
   				\STATE solve Eq.~\ref{eq:topselect} to obtain $\mat{W}^t_{L, t}$
   				\STATE $\mat{W}^t_S \leftarrow$ Selected by BFS($\mat{W}^t_{L, t}$)
   				\STATE solve $\min_{W^t}\mathcal{L}(\mat{W}^t_S; \mathcal{D}_t) + \lambda \|\mat{W}^{t}_S - \mat{W}^{t-1}_S\|^2_2$
   				\STATE Expand network $\mat{W}_{l}^t = [\mat{W}_{l}^{t-1}; \mat{W}_{l}^{\mathcal{N}}]$ for all $l$
   				\STATE solve Eq.~\ref{groupsparsity}
   				\STATE Perform Algorithm \ref{alg2} without solving Eq.~\ref{eq:l2regular} to obtain duplicated neurons
   				\STATE solve $\minimize_{\mat{W}^t}\mathcal{L}(\mat{W}^t, \mathcal{D}_t) + \mu \|\mat{W}^t\|_1 + \gamma \|\mat{W}^t\|_2$ for only duplicated neurons
   			\ENDIF
   		\STATE $\mat{W}^{t-1} \leftarrow \mat{W}^t$
   \ENDWHILE 
\end{algorithmic}
\end{algorithm}
}
\eat{
\paragraph{Preventing semantic drift with model averaging}

Thus, we instead allow the model to benefit from the later learned tasks by performing parameter averaging.

Since it would require a lot of memory to store model for each task, we instead use a moving average, storing only the latest model with averaged parameters, and then take a weighted average of it and  the model that is learned for the current task. 

figure \ref{a_model} shows intuitive understanding of moving averaging. Let $W_t$ is the all parameter for task $t$. Then the model average done by $W_t = \frac{N_{t-1}}{N_t + N_{t-1}} W_{t-1} + \frac{N_{t}}{N_t + N_{t-1}} W_t$. The task $t+1$ will starts learning from here and repeats until all series of tasks are learned. 

\setlength\parindent{6pt}
Averaging is general way of preventing a semantic drift which is catastrophic forggetting. In DC-Averaging, unlike $Freezing$ agent update all parameters including bottom and middle layers with initiated from $W_{t-1}$ parameters.
}









% In the unusual situation wheren you want a paper to appear in the
% references without citing it i the main text, use \nocite


==> expansion.tex <==
\begin{figure*}[t]
\begin{minipage}{.60\textwidth}
\small 
\begin{center}
\begin{tabular}{c c}
\hspace{-0.6in}
\includegraphics[height=2.6cm]{figure/time_performance.eps}&
%\caption{Learning time with selective retraining and unused learning time on MNIST variation dataset.}
%\label{fig:t_time}
\hspace{-0.3in}
%\includegraphics[height=2.6cm]{figure/dnn_l1_selective_perform.eps}\\
\includegraphics[height=2.6cm]{figure/selective_retraining.eps}\\
(a) Training time & (b) AUROC \\

\end{tabular}

\label{fig:selective_result}
\end{center}
\end{minipage}
\hspace{-0.6in}
\begin{minipage}{.40\textwidth}
\begin{center}
\begin{small}
\begin{tabular}{c}
\begin{tabular}{lcc}
\textbf{Models} & \textbf{AUROC} & \textbf{Capacity} \\
\hline
\hline
DNN-L2    & 0.7440$\pm$0.01 & 1 \\
DNN-L2-Selective& 0.7499$\pm$0.01 & 1 \\
DEN-Constant& 0.7580$\pm$0.01 & 1.89 \\
DEN-Dynamic& \bf 0.7684$\pm$0.01 & 1.56$\pm$0.01 \\
%\hline
\end{tabular}\\
\\
\\
(c) Expansion performance
\end{tabular}
\label{expansion_table}
\end{small}
\end{center}
\end{minipage}

\caption{\small \textbf{(a-b) Effect of selective retraining.} (a) Training time for each task measured in CPU time. (b) Average per-task performance of compared models. \textbf{(c) Expansion performance.} We report both the prediction AUROC and network capacity measured by the relative number of parameters to that of DNN-MTL on MNIST-Variance dataset. Reported numbers are mean and standard error for five random splits.}
%\vspace{-0.1in}
\end{figure*}


==> revision.tex <==
\begin{table*}[t]

\begin{minipage}{.5\textwidth}
\begin{center}
\begin{small}
\begin{tabular}{c c}
\begin{tabular}{ccc}
\textbf{Models} & \textbf{AUROC} & \textbf{Capacity} \\
\hline
\hline
DNN-STL    & 0.9993 & 10.0 \\
DNN-MTL    & 0.9991 & 1.00 \\
\hline
DEN    & \textbf{0.9982} & 1.46\\
DEN-Finetune & \textbf{0.9993} & 1.46\\
DNN-EWC    & 0.9859 & 1.00 \\
DNN-Progressive & 0.9981 & 1.61 \\
DNN    & 0.9384 & 1.00 \\
%\hline
\end{tabular}\\
(a) Permuted MNIST (T=$10$)
\end{tabular}
\label{expansion_table}
\end{small}
\end{center}
\end{minipage}
\begin{minipage}{.5\textwidth}
\begin{center}
\begin{small}
\begin{tabular}{c c}
\begin{tabular}{ccc}
\textbf{Models} & \textbf{AUROC} & \textbf{Capacity} \\
\hline
\hline
CNN-STL    & 0.9232 & 5.00 \\
CNN-MTL    & 0.8839 & 1.00 \\
\hline
DEN    & \textbf{0.9129} &  1.26 \\
DEN-Finetune & \textbf{0.9304}& 1.26\\
CNN-EWC    & 0.8540 & 1.00 \\
CNN-Progressive & 0.9044 & 1.73 \\
CNN    & 0.6327 & 1.00 \\
%\hline
\end{tabular}\\
(b) CIFAR-100 (T=$5$)
\end{tabular}
\label{expansion_table}
\end{small}
\end{center}
\end{minipage}

\caption{\small \textbf{Results on the Permuted MNIST and CIFAR-100 with AlexNet (T=$5$).} (a) Average per-task AUROC and network capacity of all models relative to MTL on Permuted MNIST. (b) AUROC and relative network capacity on CIFAR-100. Each task consists of binary classification of $20$ classes as subtasks. We used a modified AlexNet for this experiment, that has 8 layers (5 Conv layers and 3 FC layers).}
%\vspace{-0.1in}
\end{table*}

